End-to-End Referring Video Object Segmentation with Multimodal Transformers

The referring video object segmentation task (RVOS) involves segmentation of a text-referred object instance in the frames of a given video. Due to the complex nature of this multimodal task, which combines text reasoning, video understanding, instance segmentation and tracking, existing approaches typically rely on sophisticated pipelines in order to tackle it. In this paper, we propose a simple Transformer-based approach to RVOS. Our framework, termed Multimodal Tracking Transformer (MTTR), models the RVOS task as a sequence prediction problem. Following recent advancements in computer vision and natural language processing, MTTR is based on the realization that video and text can be processed together effectively and elegantly by a single multimodal Transformer model. MTTR is end-to-end trainable, free of text-related inductive bias components and requires no additional mask-refinement post-processing steps. As such, it simplifies the RVOS pipeline considerably compared to existing methods. Evaluation on standard benchmarks reveals that MTTR significantly outperforms previous art across multiple metrics. In particular, MTTR shows impressive +5.7 and +5.0 mAP gains on the A2D-Sentences and JHMDB-Sentences datasets respectively, while processing 76 frames per second. In addition, we report strong results on the public validation set of Refer-YouTube-VOS, a more challenging RVOS dataset that has yet to receive the attention of researchers. The code to reproduce our experiments is available at https://github.com/mttr2021/MTTR

==> sections/recycle_bin.tex <==
\section{Section for other stuff that we might want to use - remove later}
\ab{for now I'm using this section as a repo for small paragraphs/sentences which I might use somewhere later}

A good 3D backbone for this task would output spatio-temporal features which are rich both semantically and visually.

The scores of object queries with corresponding indices across different frames (which, similarly to VisTR \cite{wang2021vistr}, relate to the same instance) are summed. Thus, a total of $N$ scores for a total of $N$ maximum instance detections are produced for the whole video sequence.
Finally, the $T_{\mathcal{I}}$ masks relating to the detection with the highest score are selected as relating to the object referred to by $\mathcal{L}$.

Note that VisTR \cite{wang2021vistr}, whose overall instance segmentation pipeline is similar to ours, chose to employ costly 3D convolutions in their segmentation module to allow mask features from adjacent frames to reinforce each other. Unlike them, we opted to place that same computational burden at an earlier stage of our model - the backbone.
By designing our pipeline this way, and due to our specific 3D backbone selection as discussed earlier, our per-frame backbone features are temporally reinforced to begin with. This allows us to take advantage of their rich spatio-temporal features in \textit{both} the Transformer \textit{and} during the segmentation process, while settling for more efficient 2D convolutions in our spatial decoder $\mathcal{S}$. \ez{be careful with emphasizing. use it only when necessary}

\ab{I'm not sure that this next sentence is really necessary... the reasoning for this in DETR is 'we noticed it leads to better performance...'. }
Finally, note that in the matching cost $\mathcal{C}_\text{Ref}$ we use probabilities instead of log-probabilities (like in $\mathcal{L}_\text{Ref}$), following \cite{carion2020detr}.

\ab{Stuff to add if after we finish writing everything else there is still some space left:}
\begin{itemize}
\item compare to video instance segmentation methods as well, and emphasize that using SwinT instead of a regular 2D backbone (like in VisTR) also allows us to take advantage of the 3D processing in both the Transformer and the segmentation process, instead of just in the segmentation process like in VisTR
\item \ab{it could be also good to add that using I3D on datasets like refer-youtube-vos would require to run in separately on a window around each frame, which is very inefficient. contrary, since our configuration of video-swinT outputs per-frame outputs, we can just run in once per window}.
\item perhaps explain why we can't easily adapt I3D into our pipeline (first because our Transformer uses just the output of the last layer of the backbone, which would be too blurry if I3D is used, while other approaches are tailored to merge the video with the text using all of I3D's outputs. second because using I3D for refer-youtuve-vos would be highly inefficient, as it does not produce per-frame outputs, and thus we would have to run it on a temporal window per frame...)
\item mention that contrary to VisTR which conducts feature extraction frame-by-frame, we have to do so using a temporal encoder to encode actions as well as visual features.
\end{itemize}

The original architecture of Video Swin consists of 4 stages, where each stage processes the video features in a different (gradually shrinking) scale. Since our Transformer is designed to operate on input features of a single scale, we naturally tried at first using the output of the 4th stage of the backbone as input to the Transformer. Unfortunately, detection of small objects proved to be too poor using these small-scale features, which ultimately hindered our results. On the contrary, we note that using larger-scale features from an earlier layer of the backbone would lead to a significantly larger computational complexity due to the global self-attention layers found at the Transformer's encoder, as well as to losing a larger portion of the backbone's expresiveness. Ultimately, we settled on using the outputs of the 3rd stage of the network (while discarding the 4th stage altogether), as we discovered that this configuration serves as a good speed-accuracy trade-off. We further note that in this configuration the outputs of the 1st and 2nd stages of the backbone are saved for the segmentation process later on in our pipeline.

For this purpose the authors also released \textit{A2D-Sentences} and \textit{JHMDB-Sentences}, the primary benchmark datasets for the task, by providing textual annotations to the original A2D \cite{xu2015can} and JHMDB \cite{jhuang2013towards} datasets.

Recently, \citet{seo2020urvos} proposed a new RVOS dataset named Refer-YouTube-VOS, based on the original YouTube-VOS dataset \cite{xu2018youtube}. Refer-YouTube-VOS is much larger then its predecessors, contains more object categories and is more densely annotated. 

% First, action semantics (i.e. movement characteristics) should be extracted for the different instances in the video, as without them the model would not be able to effectively distinguish between similar instances with respect to the given text query \ab{here refer to the visualization in the Problem and Motivation section that we will add later}. Second, for each instance in the video precise visual characteristics (e.g. shape, size, location) should be \textit{separately} extracted for each frame. These visual features are vital for producing a sequence of accurate segmentation masks for the referred object later on. 

(this advantage is less obvious in  sparsely annotated datasets, such as A2D-Sentences \cite{gavrilyuk2018a2d}, where the backbone can be fed with a window of frames centered around each target frame). 
% Contrary to I3D, Video Swin contains just a single temporal down-sampling layer \ez{there is downsampling between blocks in swin, isn't it}, no max-pooling layers, and since it follows the general structure of the Transformer \cite{vaswani2017attention} it also contains residual connections over its attention layers. These unique characteristics make this architecture significantly less prone to I3D-like side effects. Furthermore, unlike I3D, which outputs a \textit{unified} feature map for the whole frames sequence it is fed with, Video Swin can be easily modified to output \textit{per-frame} feature maps (see \cref{subsec:bbone_implementation_details}). This makes Video Swin a much more practical choice for segmenting a full sequence of consecutive video frames as required in densely annotated datasets such as Refer-YouTube-VOS\footnote{This drawback of I3D was less obvious in the past as most methods have utilized it exclusively on the sparsely annotated A2D-Sentences dataset \cite{gavrilyuk2018a2d}. In most configurations of this sort I3D is fed with a window of frames centered around each target frame. This solution would be highly inefficient of course for segmenting an entire sequence of consecutive video frames.} \cite{seo2020urvos}) \ez{better not to use footnotes}.

\ez{notations:
\begin{itemize}
    \item Features -- $\mathcal{F}$ with index, encoded $\mathcal{F}_E^{\mathcal{V}}$ and $\mathcal{F}_E^{\mathcal{T}}$. Backbone features $\mathcal{F}_B^{1,\dots n}$
    \item Object queries $\mathcal{Q} = \qty{q}$
    \item Number of instances $N_i$
    \item Text query $\mathcal{T} = \qty{t_i}$
    \item Frames $v_i$
    \item Network parts $G_x$, e.g., $G_\text{FPN}$
    \item Number of o.q. $N_q$
\end{itemize}}

\section{additional experiments}


\paragraph{Employing 4th layer of Video SwinT.} \ab{I still haven't fixed the issue where the run in this config ignores the text loss, and so the mAP is very low even though the model does learn to segment... very strange, and hopefully I can fix this on time (if not we can just put it in the supp later I guess, we are out of space anyway...)}. \cref{tbl:ablation_block} we show that fourth block is worse.

\begin{table}
	\centering
    \setlength\extrarowheight{0.3pt}
\begin{tabular}{@{\extracolsep{4pt}}l c cc@{}} 
\toprule	 	
	\multirow{2}{*}{\textbf{Method}}  &\multicolumn{2}{c}{\textbf{IoU}} & \multirow{2}{*}{\textbf{mAP}}  \\ \cline{2-3}
    &  \textbf{Overall}   & \textbf{Mean}  & \\
\midrule	
3$^{\text{rd}}$ block &69.5&61.8&44.0\\
4$^{\text{th}}$ block &&&\\
		\bottomrule
	\end{tabular}
	%}
	\caption
		{ Block effect
		}
	\label{tbl:ablation_block}
\end{table}


Each row contains text queries followed by a sequence of frames from the corresponding video. Each text query shares the same color as the instance it describes

\paragraph{Generalization to unseen temporal contexts.}
\ab{test whether our model can generalize to longer temporal contexts than the one it was trained on (without finetunning). Can performance be improved at the cost of more computation?}

